Detecting and Mitigating Hallucinations in Machine Translation: Model Internal Workings Alone Do Well, Sentence Similarity Even Better

While the problem of hallucinations in neural machine translation has long been recognized, so far the progress on its alleviation is very little. Indeed, recently it turned out that without artificially encouraging models to hallucinate, previously existing methods fall short and even the standard sequence log-probability is more informative. It means that characteristics internal to the model can give much more information than we expect, and before using external models and measures, we first need to ask: how far can we go if we use nothing but the translation model itself ? We propose to use a method that evaluates the percentage of the source contribution to a generated translation. Intuitively, hallucinations are translations "detached" from the source, hence they can be identified by low source contribution. This method improves detection accuracy for the most severe hallucinations by a factor of 2 and is able to alleviate hallucinations at test time on par with the previous best approach that relies on external models. Next, if we move away from internal model characteristics and allow external tools, we show that using sentence similarity from cross-lingual embeddings further improves these results.

==> detection_methods_junk.tex <==
\subsection{Baseline Methods}

\paragraph{String matching.} Based on previous work\lena{which???}, we use a string-based metric, chrF++~\cite{popovic-2017-chrf} of the translation with respect to reference.\lena{any motivation?}


\paragraph{External models.} \lena{bla, bla, update}
and two metrics based on external models, COMET which is a sentence pair score trained on MT human scores \cite{rei-etal-2020-comet}; and a variation of it, COMET-QE, which does not use the reference sentence \cite{rei-etal-2020-unbabels}.

\paragraph{Internal characteristics: Seq-Logprob.}
For a trained model $P(y|x, \theta)$ and a translation~$y$, \textsf{Seq-Logprob} is the length-normalised sequence log-probability: $\frac{1}{L} \sum\limits_{k=1}^{L} \log P(y_{k} \mid y_{<k}, x, \theta)$. This is the strongest baseline according to \citet{guerreiro_hallucinations}.

\lena{separate models with seq-logprob: model internal stuff vs external models. For internal, we propose source and target contributions. For external, other representations.}


\subsection{Internal: Source and Target Contributions}

\lena{intuition: why we think source and target contributions are important. Say that it can be evaluated differently, then come to the specific method. For the method: intuition first, details later.}

\lena{reuse text below}

\paragraph{Input attributions} The ALTI+ (Aggregation of Layer-wise Tokens Attributions) method evaluates the contribution of each source and translation prefix tokens to each generated translation token. Basically, this method decomposes each transformer block into a sum of functions of individual tokens, and heuristically computes the percentage impact of each token based on this decomposition. This method predicts token alignment better than raw attention weights. In translations with artificially induced hallucinations, the average source contribution by ALTI+ has been shown to be significantly lower than in normal translations


Given a source sentence and a translation output, we want to predict if the translated output is partially or fully hallucinated. Among the different proposed measures, we use measures based on input attributions (H-ALTI+) and in learning representations with pretrained encoder-based models (H-LASER, H-LaBSE, H-XNLI).

\paragraph{H-ALTI+} We average source contribution computed with the model that has generated the translations following the ALTI+ procedure. For each target token, we compute its total source contribution as the sum of all contributions of source tokens to it; then we average it across all target tokens.


\subsection{External: Sentence Representations}


\lena{Intuition: what is our hypothesis. Something along the lines that while people looked at  MT QE, sentence representations for other tasks were largely overlooked. Which, as we will show, is a real shame.}




\paragraph{H-LASER} Consists of computing the cosine similarity of LASER2 (Hefffernan et al, 2022) source and translation sentence embeddings.
\paragraph{H-LaBSE} Consists of computing the cosine similarity of LaBSE (Feng et al, 2020) source and translation sentence embeddings.
\paragraph{H-XNLI} Consists of multiplying the probabilities of source to translation and translation to source entailments to obtain an score for hallucination. %Entailment probability predicted by a cross-lingual natural language inference model joeddav/xlm-roberta-large-xnli (a fine-tuned version of the model by Conneau et al, 2020). To obtain the score, we multiply the probabilities of source->translation and translation->source entailments.
